Can the Black Lives Matter Movement Reduce Racial Disparities? Evidence from Medical Crowdfunding

Using high-frequency donation records from a major medical crowdfunding site and careful difference-in-difference analysis, we demonstrate that the 2020 BLM surge decreased the fundraising gap between Black and non-Black beneficiaries by around 50\%. The reduction is largely attributed to non-Black donors. Those beneficiaries in counties with moderate BLM activities were most impacted. We construct innovative instrumental variable approaches that utilize weekends and rainfall to identify the global and local effects of BLM protests. Results suggest a broad social movement has a greater influence on charitable-giving behavior than a local event. Social media significantly magnifies the impact of protests.

==> Tables/tab10_main_varyingB_firstorder.tex <==
\begin{tabular}{l*{4}{c}}
\hline\hline
& \multicolumn{4}{c}{Y = Daily Number of Donors}\\
\cline{2-5}
        & (1)        & (2)         & (3)       & (4)       \\
\cline{2-5}
          & Full Sample         & B = 100 Days         & B = 50 Days       & B= 21 Days        \\
\cline{2-5}
Black_j&   -0.170\sym{***}&   -0.593\sym{***}&   -0.548\sym{***}&   -0.254\sym{*}  \\
          &  [0.051]         &  [0.072]         &  [0.105]         &  [0.154]         \\
[1em]
Black_j \times 1(t>t_{blm})&    0.223\sym{***}&    1.540\sym{***}&    1.958\sym{***}&    1.398\sym{***}\\
          &  [0.077]         &  [0.137]         &  [0.210]         &  [0.320]         \\
[1em]
Goal      &      Yes         &      Yes         &      Yes         &      Yes         \\
[1em]
Description &      Yes         &      Yes         &      Yes         &      Yes         \\
[1em]
State FE  &      Yes         &      Yes         &      Yes         &      Yes         \\
[1em]
Date FE   &      Yes         &      Yes         &      Yes         &      Yes         \\
\hline
\(N\)     &  3312525         &   689984         &   294765         &   118249         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in brackets}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}

==> Tables/tab11_donationv_varyingB.tex <==
\begin{tabular}{l*{4}{c}}
\hline\hline
& \multicolumn{4}{c}{Y = Donation Amount (\$)}\\
\cline{2-5}
        & (1)        & (2)         & (3)       & (4)       \\
\cline{2-5}
          & Full Sample         & B = 100 Days         & B = 50 Days       & B= 21 Days        \\
\cline{2-5}
Black_j&  -12.771\sym{***}&   -3.645         &   13.750         &  -14.960\sym{***}\\
          &  [2.222]         & [10.051]         & [28.694]         &  [3.905]         \\
[1em]
Black_j\times 1(t > t_{blm}) & 67.271         &  265.763         &  578.496         &   -3.700         \\
          & [71.024]         &[266.749]         &[577.891]         &  [4.177]         \\
[1em]
Goal      &      Yes         &      Yes         &      Yes         &      Yes         \\
[1em]
Description &      Yes         &      Yes         &      Yes         &      Yes         \\
[1em]
State FE \& Date FE  &      Yes         &      Yes         &      Yes         &      Yes         \\
[1em]
\hline
\(N\)     &  2911220         &   608533         &   256260         &   102719         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in brackets}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}

==> Tables/tab12_treatmentintensity_binary.tex <==
\begin{tabular}{l*{2}{c}}
\hline\hline
Full Sample & Y = Daily Number of Donors\\
\hline
\multicolumn{2}{c}{Panel (a)}\\
\hline
 Black_j\times1(t>t_{blm})&   Black_j\times1(t>t_{blm})\times\text{High Protest}\\
 0.202\sym{***}         &       0.388     \\
[1em]
  [0.042]        &  [0.379]         \\
[1em]
\hline
\multicolumn{2}{c}{Panel (b)}\\
\hline
 Black_j\times1(t>t_{blm})&   Black_j\times1(t>t_{blm})\times\text{High Gap}\\
 -0.360\sym{***}         &       1.734\sym{***}     \\
[1em]
  [0.038]        &  [0.362]           \\
[1em]

\hline
\multicolumn{2}{c}{Panel (c)}\\
\hline
 Black_j\times1(t>t_{blm})&   Black_j\times1(t>t_{blm})\times\text{High Discrimination}\\
 0.177\sym{*}         &       0.463     \\
[1em]
  [0.374]        &  [0.372]         \\
[1em]
Goal      &      Yes         \\
[1em]
Description &      Yes         \\
[1em]
State FE \& Date FE &      Yes         \\
[1em]
Zip FE    &      Yes         \\
\hline
\(N\)     &  3051974         \\
\hline\hline
\multicolumn{2}{l}{\footnotesize Standard errors in brackets}\\
\multicolumn{2}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}

==> Tables/tab13_heterogeneity_binary.tex <==
\begin{tabular}{l*{2}{c}}
\hline\hline
Full Sample & Y = Daily Number of Donors\\
\hline
\multicolumn{2}{c}{Panel (a)}\\
\hline
Black_j\times 1(t>t_{blm})&   Black_j\times 1(t>t_{blm})\times \text{More Black}\\
     0.531     &      -0.304    \\
[1em]
   [0.338]        &     [0.326]      \\
[1em]
\hline
\multicolumn{2}{c}{Panel (b)}\\
\hline
Black_j\times 1(t>t_{blm})&   Black_j\times 1(t>t_{blm})\times\text{High Income}\\
    0.134\sym{***}      &     0.523        \\
[1em]
   [0.041]       &      [0.355]      \\
[1em]

\hline
\multicolumn{2}{c}{Panel (c)}\\
\hline
Black_j\times 1(t>t_{blm})&   Black_j\times 1(t>t_{blm})\times\text{Democrats}\\
    0.112\sym{**}      &      0.392      \\
[1em]
    [0.052]       &      [0.302]       \\
[1em]
\hline
\multicolumn{2}{c}{Panel (d)}\\
\hline
Black_j\times 1(t>t_{blm})&   Black_j\times 1(t>t_{blm})\times\text{High Internet}\\
   0.547\sym{*}        &      -0.337      \\
[1em]
   [0.323]       &     [0.288]        \\
[1em]
\hline
Goal      &      Yes         \\
[1em]
Description &      Yes         \\
[1em]
State FE \& Date FE &      Yes         \\
[1em]
Zip FE    &      Yes         \\
\hline
\(N\)     &  3051974         \\
\hline\hline
\multicolumn{2}{l}{\footnotesize Standard errors in brackets}\\
\multicolumn{2}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}

==> Tables/tab14_whodonatemore.tex <==
\begin{tabular}{l*{3}{c}}
\hline\hline
 & \multicolumn{3}{c}{Y = Daily Number of Donors}\\
\hline
          &\multicolumn{1}{c}{$y_{j,t}$}&\multicolumn{1}{c}{$y_{j,t}^{ \mathcal{B}}$}&\multicolumn{1}{c}{$y_{j,t}^{W}$}\\
          \hline
          &\multicolumn{3}{c}{\textit{Panel A}: Full Sample}\\
\cline{2-4}
Black_j&   -0.238         &    0.158\sym{***}&   -0.397\sym{**} \\
          &  [0.161]         &  [0.003]         &  [0.161]         \\
[1em]
Black_j\times 1(t>t_{blm})&    0.400\sym{**} &    0.027\sym{***}&    0.373\sym{**} \\
          &  [0.190]         &  [0.004]         &  [0.189]         \\
[1em]

\cline{2-4}
& \multicolumn{3}{c}{\textit{Panel B}: Short-Term Sample} \\
\cline{2-4}

Black_j&   -0.237         &    0.158\sym{***}&   -0.395\sym{**} \\
          &  [0.158]         &  [0.003]         &  [0.157]         \\
[1em]
Black_j\times 1(t>t_{blm})&    1.070\sym{***}&    0.119\sym{***}&    0.951\sym{***}\\
          &  [0.304]         &  [0.010]         &  [0.301]         \\
\cline{2-4}
&\multicolumn{3}{c}{\textit{Panel C}: Long-Term Sample}\\
\cline{2-4}
Black_j&   -0.223         &    0.159\sym{***}&   -0.382\sym{**} \\
          &  [0.155]         &  [0.003]         &  [0.155]         \\
[1em]
Black_j\times 1(t>t_{blm})&    0.278         &    0.009\sym{**} &    0.269         \\
          &  [0.175]         &  [0.004]         &  [0.175]         \\
[1em]          
\hline
Description \& Goal &      Yes         &      Yes         &      Yes         \\
[1em]
State FE \& Date FE &      Yes         &      Yes         &      Yes         \\
[1em]
Zip FE    &      Yes         &      Yes         &      Yes         \\
\hline
\(N\)     &  3051974         &  3051974         &  3051974         \\
\hline\hline
\multicolumn{4}{l}{\footnotesize Standard errors in brackets}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}

==> Tables/tab5_main_varyingB.tex <==
\begin{tabular}{l*{4}{c}}
\hline\hline
& \multicolumn{4}{c}{Y = Daily Number of Donors}\\
\cline{2-5}
        & (1)        & (2)         & (3)       & (4)       \\
\cline{2-5}
          & Full Sample         & B = 100 Days         & B = 50 Days       & B= 21 Days        \\
\cline{2-5}
Black_j&   -0.212         &    0.034         &   -0.046         &   -0.281\sym{***}\\
          &  [0.168]         &  [0.041]         &  [0.064]         &  [0.091]         \\
[1em]
Black_j \times 1(t > t_{blm})&    0.299\sym{*}  &    0.323\sym{***}&    0.909\sym{***}&    1.455\sym{***}\\
          &  [0.163]         &  [0.058]         &  [0.093]         &  [0.155]         \\
[1em]
Goal      &      Yes         &      Yes         &      Yes         &      Yes         \\
[1em]
Description &      Yes         &      Yes         &      Yes         &      Yes         \\
[1em]
State FE \& Date FE  &       Yes         &       Yes         &      Yes         &      Yes         \\
[1em]
\hline

\(N\)     &  3312525         &   689984         &   294765         &   118249         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in brackets}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}

==> Tables/tab6_main_Bfull.tex <==
\begin{tabular}{l*{4}{c}}
\hline\hline
  Full Sample & \multicolumn{4}{c}{Y = Daily Number of Donors}\\
\cline{2-5}
        & (1)        & (2)         & (3)       & (4)       \\
\cline{2-5}
Black_j&   -0.233         &   -0.235         &   -0.212         &   -0.215         \\
          &  [0.151]         &  [0.151]         &  [0.168]         &  [0.140]         \\
[1em]
Black_j \times \textbf{1}(t\geq t_{May28})&    0.275\sym{*}  &    0.267\sym{*}  &    0.299\sym{*}  &    0.353\sym{**} \\
          &  [0.152]         &  [0.150]         &  [0.163]         &  [0.153]         \\
[1em]
Goal      &              &      Yes         &      Yes         &      Yes         \\
[1em]
Description &               &                &      Yes         &      Yes         \\
[1em]
State FE \& Date FE  &              &               &      Yes         &      Yes         \\
[1em]
Zip FE    &               &              &            &      Yes         \\
[1em]
Description $\times 1(t > t_{blm})$ &              &              &                &      Yes         \\
\hline
\(N\)     &  3313030         &  3313030         &  3312525         &  3312286         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in brackets}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}

==> Tables/tab7_main_B100.tex <==
\begin{tabular}{l*{4}{c}}
\hline\hline
  B = 100 Days       & \multicolumn{4}{c}{Y = Daily Number of Donors}\\
  \cline{2-5}
  & (1)        & (2)         & (3)       & (4)       \\
\cline{2-5}
Black_j&   -0.014         &   -0.014         &    0.034         &   -0.012         \\
          &  [0.040]         &  [0.040]         &  [0.041]         &  [0.047]         \\
[1em]
Black_j \times 1(t>t_{blm})&    0.326\sym{***}&    0.323\sym{***}&    0.329\sym{***}&    0.421\sym{***}\\
          &  [0.059]         &  [0.059]         &  [0.058]         &  [0.064]         \\
[1em]
Goal      &                &      Yes         &      Yes         &      Yes         \\
[1em]
Description &               &               &      Yes         &      Yes         \\
[1em]
State FE \& Date FE &                &              &      Yes         &      Yes         \\
[1em]
Zip FE    &                &                &              &      Yes         \\
[1em]
Description $\times 1(t > t_{blm})$ &                &                &              &      Yes         \\
\hline
\(N\)     &   685615         &   685615         &   685615         &   684930         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in brackets}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}

==> Tables/tab8_main_B21.tex <==
\begin{tabular}{l*{4}{c}}
\hline\hline
  B = 21 Days       & \multicolumn{4}{c}{Y = Daily Number of Donors}\\
  \cline{2-5}
  & (1)        & (2)         & (3)       & (4)       \\
\cline{2-5}
Black_j&   -0.384\sym{***}&   -0.373\sym{***}&   -0.276\sym{***}&   -0.063         \\
          &  [0.089]         &  [0.089]         &  [0.091]         &  [0.134]         \\
[1em]
Black_j\times 1(t>t_{blm})&    1.415\sym{***}&    1.413\sym{***}&    1.446\sym{***}&    1.226\sym{***}\\
          &  [0.158]         &  [0.158]         &  [0.157]         &  [0.162]         \\
[1em]
Goal      &                &      Yes         &      Yes         &      Yes         \\
[1em]
Description &              &               &      Yes         &      Yes         \\
[1em]
State FE \& Date FE  &                &               &      Yes         &      Yes         \\
[1em]
Zip FE    &              &                &               &      Yes         \\
[1em]
Description $\times 1(t > t_{blm})$  &               &               &               &      Yes         \\
\hline
\(N\)     &   114869         &   114869         &   114869         &   113594         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in brackets}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}

==> Tables/tab9_main_varyingB_jfe.tex <==
\begin{tabular}{l*{4}{c}}
\hline\hline
& \multicolumn{4}{c}{Y = Daily Number of Donors}\\
\cline{2-5}
        & (1)        & (2)         & (3)       & (4)       \\
\cline{2-5}
          & Full Sample         & B = 100 Days         & B = 50 Days       & B= 21 Days        \\
\cline{2-5}
Black_j&   -0.734         &   -0.155\sym{**} &   -0.099         &    0.013         \\
          &  [0.810]         &  [0.079]         &  [0.108]         &  [0.150]         \\
[1em]
Black_j\times 1(t>t_{blm})&    0.714         &    0.422\sym{***}&    0.588\sym{***}&    0.609\sym{***}\\
          &  [0.611]         &  [0.074]         &  [0.105]         &  [0.152]         \\
[1em]
Project FE      &      Yes         &      Yes         &      Yes         &      Yes         \\
\hline
\(N\)     &   508294         &   220441         &   120581         &    63471         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in brackets}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}

==> Tables/tab_reg_localprotest_OLS_national100.tex <==
\begin{tabular}{@{}lccccc@{}}
\hline \hline
 & \multicolumn{5}{c}{$y$ =   Num. Daily Donation} \\ \cmidrule(l){2-6} 

 & (1) & (2) & (3) & (4) & (5) \\ \cmidrule(l){2-6} 
$Black_j \times protest_{ct}$ & 0.139** & -1.084 & -0.247 & 0.369** & 0.172*** \\
 & (2.54) & (-1.15) & (-0.80) & (2.45) & (3.05) \\
 &  &  &  &  &  \\
$Black_j \times Protest_{-ct}$ & 0.018*** & 0.034* & 0.025** & 0.000 & 0.014 \\
 & (2.59) & (1.85) & (2.10) & (0.01) & (1.07) \\
 &  &  &  &  &  \\

 \hline
 Description \& Goal & Yes & Yes & Yes & Yes & Yes \\
County & Yes & Yes & Yes & Yes & Yes \\
County $\times$ Black & Yes & Yes & Yes & Yes & Yes \\
County $\times \textbf{1}(t>t_{May27})$ & Yes & Yes & Yes & Yes & Yes \\
 &  &  &  &  &  \\
Sample & Full & Quantile 1 & Quantile 2 & Quantile 3 & Quantile 4 \\
Observations & 605888 & 155369 & 178365 & 125383 & 146698 \\ 
\\

\hline \hline
t statistics in brackets &  &  &  &  &  \\
*   p\textless{}0.10  ** p\textless{}0.05  *** p\textless{}0.01 &  &  &  &  & 

\end{tabular}
